Brain-inspired reverse adversarial examples

A human does not have to see all elephants to recognize an animal as an elephant. On contrast, current state-of-the-art deep learning approaches heavily depend on the variety of training samples and the capacity of the network. In practice, the size of network is always limited and it is impossible to access all the data samples. Under this circumstance, deep learning models are extremely fragile to human-imperceivable adversarial examples, which impose threats to all safety critical systems. Inspired by the association and attention mechanisms of the human brain, we propose reverse adversarial examples method that can greatly improve models' robustness on unseen data. Experiments show that our reverse adversarial method can improve accuracy on average 19.02% on ResNet18, MobileNet, and VGG16 on unseen data transformation. Besides, the proposed method is also applicable to compressed models and shows potential to compensate the robustness drop brought by model quantization - an absolute 30.78% accuracy improvement.

==> ProbStatement_old.tex <==
\section{Proposed brain-inspired calibrater}


%Adversarial attacks change the classification results of models by either maximizing the loss with respect to the true label or minimizing the loss respect to the target label, which used to any label other than the true one.

%In this work, we show that it is actually useful to minimize the loss of the model with respect to the true label by optimizing the perturbation $\theta$.  We call the modified inputs and the perturbation reverse adversarial examples and benign perturbation respectively. To utilize the benign perturbation, we propose a generative model called calibrater. 

Figure \ref{fig: Overview} shows an overview of the proposed framework. Traditional deployment process for deep learning models usually starts with training a model in one specific training dataset, which is assumed to be close to the application scenes. Once the model is trained, a common practice is to use the same dataset for model compression training\cite{zhou2017incremental,han2015deep}. After that, models are deployed in hardware such as ASIC. However, the real world is complicated - the assumption that the training data and data in application scenes being independently and identically distributed rarely holds. Scenes might change: for self-driving data collected in a city that is always sunny is very different from those of a city that rains a lot.
In such cases, the performance degradation occurs. 
In order to compensate the performance degradation, the traditional approach is either adding the new data to fine-tune the original model or training a completely new model that is only good for the new scene. In both cases it is costly to retrain the model. This issue scales up quickly with when the size of main models and the number of deployed devices increase.

The proposed method approaches this issue in a different direction: instead of asking models to fit every possible scene, it's more feasible to train a light-weight calibrater which is trained with new data that is capable of converting new data to data that the deployed models understand. Using this approach, models can work correctly without the need to be aware of change of scenes.
Figure~\ref{fig: Overview} demonstrates the proposed deployment process. 
In traditional deployment process, once new scenes are encountered and performance degradation is observed, the main model is then 
retrained with new data, which consumes significant amount of resources as well as delaying the deployment.
However, in the proposed deployment process, the main model can be fixed, and only the light-weight generative calibrater is re-trained.
The generative model is extremely light-weight which makes it possible to run in an ARM embedded processor. 
Once the deployed device is switched for different
scenarios, it is very flexible to update the calibrater running on ARM, rather than
the main model running on ASIC.
In this way, the proposed calibrater serves as a pre-processing unit for a deep learning model.
\subsection{Notation}
We use $f(.)$ to denote a neural network and $c(.)$ to denote the classification result of the neural network, where $c(x) = argmax(f(x))$ for input $x$. A neural network that's trained in $x$ denotes $f^*{(x)}$, which is considered optimal for data $x$. In case for new data $x'$, we consider $f^*(x')$ gives sub-optimal classification results. 
\subsection{Brain-inspired calibrater}

We now explain the relationship between adversarial examples and proposed reverse adversarial examples. Typical adversarial attack methods searches for $\delta$ so that $c(x+\delta) \neq c^*{(x)}$ by maximizing the classification loss on $f(x+\delta)$ or minimizing $||\delta||$~\cite{goodfellow2014explaining,kurakin2016adversarial,carlini2017towards}.  By reversing the goal of adversarial attack and borrow the idea from attention mechanism in brain, we set the goal of generative model to be generating a $\delta$ so that $c({x'}\cdot\delta) = c^*(x')$ by minimizing classification loss on $f({x'}\cdot\delta)$. 
What differs our reverse adversarial examples methodology from adversarial examples methodology are two-folds: (i) Given $x'$, which the main model is not optimal for, we perform reverse adversarial attack by asking the generative model to output  $\delta$ to minimize classification loss of the main model $f({x'}\cdot\delta)$. (ii) While adversarial attacks merge perturbation into input x by addition, we instead apply multiplication to mimic the attention mechanism in brain. 
Therefore, the overall objective function for the generative model is:
\begin{align}\label{eq: fx}
\small
%L(\mathbf{x}_i\cdot G(\mathbf{x}_i),\mathbf{y}_i,\theta_{G}) = 1 - F(\mathbf{x}_i \cdot  G(\mathbf{x}_i),\theta_{M})_{t_i} ,
L_{G} = max(\mathbf{y}_i) - F(\mathbf{x}_i \cdot  G(\mathbf{x}_i,\theta_{G}), \theta_{M})_{j} ,
\end{align}
where $j = argmax (\mathbf{y}_i)$ for ground truth $\mathbf{y}_i$.
\begin{algorithm}[h]  
\caption{Training for proposed calibrater}  
\begin{algorithmic}[1]  
\Require{Dataset A, main model M, dataset B, generative model G, optimizer Opt}
\State{Train a model M in dataset A.}
%\For{batch in Dataloader(A)} \State // \emph{Can be avoided if M is already trained}
%\State{data,target = getData(batch)}
%\State{output = M.getOutput(data)}
%\State{loss = CrossEntropy(output,target)}
%\State{grad = Opt.getGradient(loss)}
%\State{weightUpdate(M,grad)}
%\EndFor
\State{$M.backward(False)$} \State // \emph{Disables the backpropagation of M}
\For{batch in Dataloader(dataset B)}
\State{$data,target = getData(batch)$}
\State{$\delta = G.getOutput(data)$}
\State{$F = M.getSoftMaxOutputs(data \cdot \delta)$}
\State{$index = argmax(target)$}
\State{$loss = 1- F[index]$}
\State{$grad = Opt.getGradient(loss)$}
\State{$weightUpdate(G,grad)$}
\EndFor
\end{algorithmic}  
\label{train}
\end{algorithm} 


Algorithm \ref{train} describes the training procedure for the proposed calibrater. We assume that the main model M is already trained in dataset A and will be deployed in dataset B. To simulate the cases where it is not feasible to retrain model M, backward propagation for M is disabled. The calibrater leverages the inference result of model M for training.

%\For {$i$ in number of layers in G do}


%\State{index = argmax(target)}
%\State{loss = 1- F[index]}
%\State{grad = Opt.getGradient(loss)}
%\State{weightUpdate($W_i$,grad)}
%\EndFor


%By chain rule, we know that the gradient of loss with respect to the perturbation is :
%\begin{align}\label{eq: chain_rule}
%\small
%\frac {\partial L} {\partial \mathbf{\delta}} = \frac {\partial L} {\partial \mathbf {x'}} \cdot \frac {\partial \mathbf {x'}} {\partial \mathbf{\delta}}
%\end{align}
%We denote \emph{x'} as the perturbed input. 

%For case 1:  $x' = x + \mathbf{\delta} $, $\frac {\partial \mathbf {x'}} {\partial \mathbf{\delta}} = 1$;

%For case 2: $x' = x \cdot \mathbf{\delta} $, $\frac {\partial \mathbf {x'}} {\partial \mathbf{\delta}} = x$




